Distributed Iterative CT Reconstruction using Multi-Agent Consensus Equilibrium

Model-Based Image Reconstruction (MBIR) methods significantly enhance the quality of computed tomographic (CT) reconstructions relative to analytical techniques, but are limited by high computational cost. In this paper, we propose a multi-agent consensus equilibrium (MACE) algorithm for distributing both the computation and memory of MBIR reconstruction across a large number of parallel nodes. In MACE, each node stores only a sparse subset of views and a small portion of the system matrix, and each parallel node performs a local sparse-view reconstruction, which based on repeated feedback from other nodes, converges to the global optimum. Our distributed approach can also incorporate advanced denoisers as priors to enhance reconstruction quality. In this case, we obtain a parallel solution to the serial framework of Plug-n-play (PnP) priors, which we call MACE-PnP. In order to make MACE practical, we introduce a partial update method that eliminates nested iterations and prove that it converges to the same global solution. Finally, we validate our approach on a distributed memory system with real CT data. We also demonstrate an implementation of our approach on a massive supercomputer that can perform large-scale reconstruction in real-time.

==> mace_desc_prev.tex <==
{\bf No:  the key idea of CE is to formulate the problem as an equilibrium problem among agents.  
In the case of an optimization, the agents are typically proximal maps or approximations to them.}
Similar to the broad family of proximal-splitting algorithms, the key idea of the Multi-Agent CE framework \cite{Buzzard2018CE}, is to associate a \emph{proximal map} with each function $f_i, i=1,...,N$, of equation (\ref{eq:consensus_prob}).
We define $F_i(\cdot \ ; \sigma) : \RR^n \rightarrow \RR^n$, the proximal map of function $f_i:\RR^n \rightarrow \RR$, as
\begin{align}
F_i(x ; \sigma) = \argmin_{z \in \RR^n} \left\{f_i(z) + \frac{\|z-x\|^2}{2 \sigma^2} \right\}.
\label{eq:prox_F}
\end{align}
We more broadly refer to each of these individual proximal maps, $F_i, i=1,...,N$, as an \emph{agent}.
In broad terms, an agent could even be a non-proximal operator such as a neural network.
Importantly, the MACE framework specifies a general system of equations involving $N$ different agents, which upon solving provides us the consensus solution. 
Further, Buzzard et al in \cite{Buzzard2018CE} suggest various techniques to solve the MACE system of equations in a distributed manner.
While some of these distributed techniques closely resemble proximal-splitting algorithms, \cite{Buzzard2018CE} further includes advanced methods that can handle novel consensus formulations, wherein one or more agents in the system are non-proximal operators, or even mildly expansive operators.\\     

Prior to further discussion of the MACE framework, we introduce the following notations for the onward sections of this paper: 
\begin{itemize}
\item
We use \textbf{bold} notation to denote a tall vector consisting of $N$ individual vectors, each $\in \RR^n$. 
For example, $\v \in \RR^{nN}$ denotes a tall vector, where $v_i \in \RR^n, \ i=1,...,N$ are the individual components of $\v$.
\item
We use the \textbf{bold} notation with a ``bar" superscript to represent component-wise averaging operation on a tall vector.
For example, for $\v \in \RR^{nN}$, $\bar{\v} \in \RR^n$ is given by 
$$
\bar{\v} = (1/N)\sum_{i=1}^N v_i.
$$
\item
We use the notation $\hat{x}$ to denote a tall vector obtained by vertically stacking $x \in \RR^n$ N times.\\
\end{itemize}

% \noindent
% **System of equations (with theorem) and its compact representation (with theorem)**\\
% ** A specific case of Mann iterations $\rho =0.5$ is the distributed MLEM alg** \\

In the specific case of $N$ different proximal agents $F_1, \cdots, F_N$, the system of equations specified by the MACE framework is given by
\begin{align}
    F_i(x^*-u_i^*; \sigma)&=x^*, i=1,...,N, \label{eq:CEsys_F}\\
    \bar{\u}^*&=0 , \label{eq:CEsys_u} 
\end{align}
where $x^* \in \RR^n$ and $ \u^* \in \RR^{nN}$.
Importantly, for any non-zero choice of $\sigma$, the pair $(x^*, \u^*)$ represents the solution to the MACE system of equations, and further, $x^*$ is the true consensus solution to the problem represented by equation (\ref{eq:consensus_prob}).
This result is summarized by the below theorem.

\begin{theorem} \label{thm:CE_conditions}
Let $f_i: \RR^n \rightarrow \RR, i=1,...,N$, each represent a proper convex function, and define $f = \sum_{i=1}^N f_i$.
Let $F_i(\cdot ; \sigma):\RR^n \rightarrow \RR^n$ represent the proximal map of $f_i$ as defined by equation (\ref{eq:prox_F}).
Then the set of solutions $(x^*, \u^*)$ to the MACE system of equations defined by (\ref{eq:CEsys_F}) and (\ref{eq:CEsys_u}) is exactly the same set of solutions to the consensus problem of (\ref{eq:consensus_prob}).
\end{theorem}

\begin{proof}
This is a specific case of Theorem 1 proved in \cite{Buzzard2018CE}.
\end{proof}

The MACE system of equations represented by (\ref{eq:CEsys_F}) and (\ref{eq:CEsys_u}) can be expressed in a more compact form.
Let us define the stacked operators $\F:\RR^{nN}\rightarrow \RR^{nN}$ and $\G:\RR^{nN}\rightarrow \RR^{nN}$ as
\begin{align}
\F(\v) = \left(
\begin{array}{c}
F_1(v_1; \sigma) \\
\vdots  \\
F_N(v_N; \sigma)
\end{array}
\right),
\text{ and, }
\G(\v) = \left(
\begin{array}{c}
\bar{\v} \\
\vdots  \\
\bar{\v}
\end{array}
\right).
\label{eq:FG_operators}
\end{align}
As per our prescribed notation, let $\hat{x}^*$ represent $N$ stacked copies of $x^*$. 
Let us define $\v^* \in \RR^{nN}$ as
$$
\v^* = \hat{x}^* - \u^*. \label{eq:vdef}
$$
Note that $\bar{\v}^*=x^*$ as a consequence of equation (\ref{eq:CEsys_u}).
So, the MACE system of equations can alternately be represented as
\begin{align}
    \F(\v^*) = \G(\v^*).
\label{eq:CEsys_compact}
\end{align}
Note that once we determine $\v^*$ that satisfies the above condition, we easily obtain $x^*$, the solution to the consensus problem of equation (\ref{eq:consensus_prob}), as $x^*=\bar{\v}^*$.

One specific method from \cite{Buzzard2018CE} that we use to determine $\v^*$ is by re-formulating the problem of (\ref{eq:CEsys_compact}) as determining the \emph{fixed-point} of a particular map involving operators $\F$ and $\G$. 
This approach is summarized by the following theorem.

\begin{theorem} \label{thm:CE_fixed}
Let the operators $\F$ and $\G$ on $\RR^{nN} \rightarrow \RR^{nN}$ be defined as in equation (\ref{eq:FG_operators}).
Let $\v^* \in \RR^{nN}$ and define $\w^*=(2\G-\I)\v^*$.
Then, $\v^*$ is a solution to equation (\ref{eq:CEsys_compact}) if and only if $\w^*$ satisfies the condition
\begin{align}
(2\F-\I)(2\G-\I)\w^* = \w^*.
\label{eq:w*_fixed_pt}
\end{align}
Further, the pair $(x^*, \u^*) \in \RR^n \times \RR^{nN}$ that solves the MACE system of equations in (\ref{eq:CEsys_F}) and (\ref{eq:CEsys_u}) can be obtained from $\w^*$ as  $(\bar{\w}^*,\w^*-\G\w^*)$.
\end{theorem}

\begin{proof}
While the proof is available in \cite{Buzzard2018CE}, we provide the key ideas in Appendix A.
\end{proof}

The above theorem states that we can determine the solution to the consensus problem of (\ref{eq:consensus_prob}) by finding $\w^* \in \RR^{nN}$, the fixed-point of a specific map $\T:\RR^{nN} \rightarrow \RR^{nN}$, where $\T$ is defined as $\T=(2\F-\I)(2\G-\I)$.
One particular method to evaluate $\w^*$ is the Mann iteration \cite{ParikhProximal}.
In this iterative approach, we start with any initial guess of $\w^*$, say $\w^{(0)}$, and then iteratively update our estimate of $\w^*$ as the weighted average between $\T \w^{(k)}$ and $\w^{(k)}$, $k \ge 0$, as shown below.
\begin{equation}
\w^{(k+1)} = \rho (2\F-\I)(2\G-\I)\w^{(k)} + (1-\rho)\w^{(k)}, k\ge 0.
\label{eq:Mann}
\end{equation}
It is worth noting that this approach is guaranteed to converge to the fixed-point because the map $\T$ is non-expansive.
Since proximal maps $F_i, i=1,...,N$ belong to a special class of operators called \emph{resolvent} operators \cite{ParikhProximal},  both $F_i$ as well as $2F_i-I$ are non-expansive.
Consequently, $2\F-\I$ is non-expansive.
Since $\T$ is the composition of two non-expansive maps $2\F-\I$ and $2\G-\I$, $\T$ is non-expansive.

Importantly, note that operator $\F$, which in practice constitutes the bulk of computation in (\ref{eq:Mann}), is a parallel operator. 
This is because $\F(\v)$ can be executed by $N$ parallel nodes of a distributed memory system, where the $i$-th node stores $v_i$, the $i$-th component of $\v$, and computes $F_i(v_i)$, the $i$-th proximal map with $v_i$ as input.
Further, note that $\G$ can be interpreted as a centralized merge and broadcast operator. 
This is because $\G(\v)$ first evaluates $\bar{\v}$, the average of the $N$ components of $\v$, and then stacks $N$ copies of $\bar{\v}$ vertically.
The averaging operation requires centralized communication between $N$ nodes, since $v_i$ for each $i=1,...,N$ is stored on a different node.
The vertical stacking operation  resembles broadcasting the averaged result from a central node to the $N$ individual nodes.
Since $\G$ typically has limited overhead in comparison to parallel operator $\F$, the algorithm specified by (\ref{eq:Mann}) is parallel.

Importantly, in Appendix A, we show that the distributed MLEM approach of \cite{Cui} is a particular case of our approach described by equation (\ref{eq:Mann}).
More specifically, when $\rho=0.5$, our approach is equivalent to the approach in \cite{Cui}.
We verify in our experiments that a better choice of $\rho$ can significantly improve algorithmic convergence.
Across multiple datasets used in this paper, $\rho=0.8$ seems to result in best algorithmic convergence.
